MobileVOS: Real-Time Video Object Segmentation Contrastive Learning meets Knowledge Distillation

This paper tackles the problem of semi-supervised video object segmentation on resource-constrained devices, such as mobile phones. We formulate this problem as a distillation task, whereby we demonstrate that small space-time-memory networks with finite memory can achieve competitive results with state of the art, but at a fraction of the computational cost (32 milliseconds per frame on a Samsung Galaxy S22). Specifically, we provide a theoretically grounded framework that unifies knowledge distillation with supervised contrastive representation learning. These models are able to jointly benefit from both pixel-wise contrastive learning and distillation from a pre-trained teacher. We validate this loss by achieving competitive J&F to state of the art on both the standard DAVIS and YouTube benchmarks, despite running up to 5x faster, and with 32x fewer parameters.

==> tables/aspp.tex <==
TODO

==> tables/data_efficiency_davis16.tex <==
\begin{tabular}{cccc}
    \toprule
    \textbf{Training data} & $\JandF$ & $\J$ & $\F$ \\
    \midrule
    DAVIS only & - & - & - \\
    DAVIS+YouTubeVOS only & - & - & - \\
	Static+DAVIS+YouTubeVOS & - & - & - \\
% 	Static+BL30K+DAVIS+YouTubeVOS & - & - & - \\
    \bottomrule
\end{tabular}

==> tables/data_efficiency_davis17.tex <==
\begin{tabular}{cccc}
    \toprule
    \textbf{Training data} & $\JandF$ & $\J$ & $\F$ \\
    \midrule
    DAVIS only & - & - & - \\
    DAVIS+YouTubeVOS only & - & - & - \\
	Static+DAVIS+YouTubeVOS & - & - & - \\
% 	Static+BL30K+DAVIS+YouTubeVOS & - & - & - \\
    \bottomrule
\end{tabular}

==> tables/mobile.tex <==

\begin{tabular}{ccccc}
    \toprule
    \textbf{Architecture} & Segmenter & Value Encoder \\
    \midrule
    %\multirow{3}{*}{\small\textbf{ResNet18}}
    

    \textbf{STCN} & 510.0 & 271.0 \\
    \textbf{MobileVOS} & 45.8 & 28.2 \\
    \textbf{MobileVOS + ASPP} & 53.3 & 28.2 \\
    
    \bottomrule
\end{tabular}

==> tables/model_soup.tex <==

\begin{tabular}{cccc}
    \toprule
    Model & DAVIS16 & DAVIS17 & YoutubeVOS \\
    % $\omega$ & DAVIS16 & DAVIS17 \\
    \midrule

    $0.0$ & \textbf{91.0} & 83.1 & \textbf{82.3} \\

    	$0.2$ & 90.6 & \underline{83.7} & 81.3 \\

    	$0.8$ & 90.2 & 83.4 & \underline{81.5} \\

    	$1.0$ & \underline{90.9} & \textbf{84.2} & 81.1 \\

    \bottomrule
\end{tabular} 


==> tables/multi_scale.tex <==
\begin{tabular}{cccccc}
    \toprule
    & \textbf{\# Scales} & $\JandF$ & $\J$ & $\F$ \\
    \midrule
    \multirow{3}{*}{\small\textbf{ResNet18}}
    
    & 1 & - & - & - \\
	& 2 & - & - & - \\
	& 4 & - & - & - \\

    \bottomrule
\end{tabular}

==> tables/performance.tex <==
\resizebox{1.\linewidth}{!}{
\centering
\begin{tabular}{lccc}
    \toprule
    Method & Params(M) &     
    \begin{tabular}{c}
        FPS \\
        \small\textit{NVIDIA A40}
    \end{tabular} &
    \begin{tabular}{c}
        FPS \\
        \small\textit{NVIDIA 1080Ti}
    \end{tabular} \\
    \midrule
    
    % Memory USAGE DAVIS17: 
    % FPS: 
    STM~\cite{oh2019video} & 38.9 & 8.9$\rightarrow$6.6 & {\color{red} over GPU (11GB) limit} \\
    
    GSFM~\cite{xie2021efficient} & 67.0 & 17.0$\rightarrow$9.6 & 7.5$\rightarrow$3.1 \\

    STCN~\cite{cheng2021rethinking} & 54.4 & 32.3$\rightarrow$19.2 & 16.3$\rightarrow$6.5 \\
    
    RDE-VOS~\cite{xie2021efficient} & 64.0 & 30.6$\rightarrow$33.8 & 14.7$\rightarrow$ 14.5 \\
    
    XMem~\cite{cheng2022xmem} & 62.2 & 38.6$\rightarrow$39.9 & 12.6$\rightarrow$12.7 \\
        
    \midrule
    
    MobileVOS &  &  \\
	\footnotesize ResNet18 & 8.1 & \textbf{67.0}$\rightarrow$70.0 & 52.6$\rightarrow$54.1 \\
	
    \footnotesize MobileNetV2 & 2.5 & 50.7$\rightarrow$65.7 & 62.2$\rightarrow$63.8 \\

	\footnotesize $\rotatebox[origin=c]{180}{$\Lsh$}$ wo/ ASPP  & \textbf{1.9} & 61.7$\rightarrow$\textbf{84.8} & \textbf{67.2}$\rightarrow$\textbf{69.3} \\
    \bottomrule
\end{tabular}}

==> tables/queue_sizes.tex <==
\begin{tabular}{lc}
    \toprule
    Queue size & $\JandF$ \\
    \midrule
    1 (first) & 82.0 \\
    1 (latest) & 60.1 \\
    2 & 90.1 \\
    $\infty$ & 90.2 \\
    \bottomrule
\end{tabular}
